How are Diverse End-user Human-centric Issues Discussed on GitHub?

Many software systems fail to meet the needs of the diverse end-users in society and are prone to pose problems, such as accessibility and usability issues. Some of these problems (partially) stem from the failure to consider the characteristics, limitations, and abilities of diverse end-users during software development. We refer to this class of problems as human-centric issues. Despite their importance, there is a limited understanding of the types of human-centric issues encountered by developers. In-depth knowledge of these human-centric issues is needed to design software systems that better meet their diverse end-users' needs. This paper aims to provide insights for the software development and research communities on which human-centric issues are a topic of discussion for developers on GitHub. We conducted an empirical study by extracting and manually analysing 1,691 issue comments from 12 diverse projects, ranging from small to large-scale projects, including projects designed for challenged end-users, e.g., visually impaired and dyslexic users. Our analysis shows that eight categories of human-centric issues are discussed by developers. These include Inclusiveness, Privacy & Security, Compatibility, Location & Language, Preference, Satisfaction, Emotional Aspects, and Accessibility. Guided by our findings, we highlight some implications and possible future paths to further understand and incorporate human-centric issues in software development to be able to design software that meets the needs of diverse end users in society.

==> Tables/Results.tex <==
\begin{table*}[]
\centering
\caption{Number (\#) and percentage (\%) of human-centric issues in different projects}
\label{tbl:results}
{\scriptsize
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
                         & \multicolumn{2}{c|}{\textbf{Inclusiveness}} & \multicolumn{2}{c|}{\textbf{Privacy/security}} & \multicolumn{2}{c|}{\textbf{Compatibility}} & \multicolumn{2}{c|}{\textbf{Location/Language}} & \multicolumn{2}{c|}{\textbf{Preference}} & \multicolumn{2}{c|}{\textbf{Satisfaction}} & \multicolumn{2}{c|}{\textbf{Emotional aspects}} & \multicolumn{2}{c|}{\textbf{Accessibility}} \\ \hline
\textbf{Project}         & \textbf{\#}             & \textbf{\%}            & \textbf{\#}              & \textbf{\%}              & \textbf{\#}             & \textbf{\%}            & \textbf{\#}               & \textbf{\%}              & \textbf{\#}           & \textbf{\%}           & \textbf{\#}            & \textbf{\%}            & \textbf{\#}               & \textbf{\%}              & \textbf{\#}             & \textbf{\%}            \\ \hline
\textbf{Firefox-ios}     & 3                       & 0.82                   & 6                        & 1.63                     & 5                       & 1.36                   & 1                         & 0.27                     & 14                    & 3.81                  & 10                     & 2.72                   & 3                         & 0.82                     & 5                       & 1.36                   \\ \hline
\textbf{Cwa-app-ios}     & 14                      & 4.33                   & 11                       & 3.41                     & 13                      & 4.02                   & 18                        & 5.57                     & 5                     & 1.55                  & 17                     & 5.26                   & 3                         & 0.93                     & 4                       & 1.24                   \\ \hline
\textbf{Cwa-app-android} & 3                       & 1.66                   & 21                       & 11.60                    & 10                      & 5.52                   & 19                        & 10.50                    & 6                     & 3.31                  & 11                     & 6.08                   & 1                         & 0.55                     & 1                       & 0.55                   \\ \hline
\textbf{Healthchecks}    & 1                       & 0.34                   & 5                        & 1.71                     & 0                       & 0.00                   & 5                         & 1.71                     & 11                    & 3.75                  & 8                      & 2.73                   & 2                         & 0.68                     & 2                       & 0.68                   \\ \hline
%\textbf{Pedometer}       & 0                       & 0.00                   & 1                        & 0.63                     & 1                       & 0.63                   & 5                         & 3.13                     & 2                     & 1.25                  & 6                      & 3.75                   & 1                         & 0.63                     & 1                       & 0.63                   \\ \hline
\textbf{Mobile-ios}      & 2                       & 5.88                   & 4                        & 11.76                    & 4                       & 11.76                  & 1                         & 2.94                     & 6                     & 17.65                 & 5                      & 14.71                  & 0                         & 0.00                     & 0                       & 0.00                   \\ \hline
\textbf{Mobile-android}  & 0                       & 0.00                   & 15                       & 32.61                    & 1                       & 2.17                   & 0                         & 0.00                     & 4                     & 8.70                  & 6                      & 13.04                  & 1                         & 2.17                     & 0                       & 0.00                   \\ \hline
\textbf{Total}           & 23                      & 1.64                   & 63                       & 4.49                     & 34                      & 2.42                   & 49                        & 3.49                     & 48                    & 3.42                  & 63                     & 4.49                   & 11                        & 0.78                     & 13                      & 0.93                   \\ \hline
\end{tabular}
}
\end{table*}
